ACE: A Cardinality Estimator for Set-Valued Queries

Cardinality estimation is a fundamental functionality in database systems. Most existing cardinality estimators focus on handling predicates over numeric or categorical data. They have largely omitted an important data type, set-valued data, which frequently occur in contemporary applications such as information retrieval and recommender systems. The few existing estimators for such data either favor high-frequency elements or rely on a partial independence assumption, which limits their practical applicability. We propose ACE, an Attention-based Cardinality Estimator for estimating the cardinality of queries over set-valued data. We first design a distillation-based data encoder to condense the dataset into a compact matrix. We then design an attention-based query analyzer to capture correlations among query elements. To handle variable-sized queries, a pooling module is introduced, followed by a regression model (MLP) to generate final cardinality estimates. We evaluate ACE on three datasets with varying query element distributions, demonstrating that ACE outperforms the state-of-the-art competitors in terms of both accuracy and efficiency.

==> command.tex <==
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{property}{Property}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{observation}{Observation}

%=============defined for convenience====
\long\def\comment#1{}
\newcommand{\stitle}[1]{\vspace{1ex}\noindent{{\bf#1}}}
\newcommand{\sstitle}[1]{\vspace{1ex}\noindent{\underline{\textit{#1}}}}
% \newcommand{\sstitle}[1]{\vspace{1ex}\noindent{{\textit{#1}}}}
% \newcommand{\ssstitle}[1]{\vspace{1ex}\noindent{\underline{\textit{#1}}}}
\newcommand{\ssstitle}[1]{\vspace{1ex}\noindent{\textit{#1}}}

\newcommand{\kw}[1]{{\ensuremath {\mathsf{#1}}}\xspace}
\newcommand{\bkw}[1]{{\ensuremath {\mathsf{\textbf{#1}}}}\xspace}
\newcommand{\kwnospace}[1]{{\ensuremath {\mathsf{#1}}}}
\newcommand{\proofsketch}{\vspace*{-1ex} {\sc Proof Sketch. }}
\newcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}}
\newcommand{\code}[1]{\texttt{#1}}

%=============defined for reference======
\newcommand{\reffig}[1]{Figure~\ref{fig:#1}}
\newcommand{\refsec}[1]{Section~\ref{sec:#1}}
\newcommand{\reftab}[1]{Table~\ref{tab:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{alg:#1}}
\newcommand{\refeq}[1]{Equation~\ref{eq:#1}}
\newcommand{\refdef}[1]{Definition~\ref{def:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{thm:#1}}
\newcommand{\reflem}[1]{Lemma~R\ref{lem:#1}}
\newcommand{\refrem}[1]{Remark~\ref{rem:#1}}
\newcommand{\refcoro}[1]{Corollary~\ref{coro:#1}}
\newcommand{\refex}[1]{Example~\ref{ex:#1}}
\newcommand{\refppt}[1]{Property~\ref{ppt:#1}}

%=============for figures and tables=======
\newcommand{\topcaption}{%
	\setlength{\abovecaptionskip}{0.01cm}%
	\setlength{\belowcaptionskip}{0.01cm}%
	\caption}
	
%=============defined for StructSim======
% \newcommand{\Sim}{\kw{Sim}}
% \newcommand{\Sim}{\Gamma}
\newcommand{\tc}{\code{TC}-\code{build}}
\newcommand{\tcxs}{\code{TC}-\code{build}\xspace}
\newcommand{\tcpara}{\code{TC}-\code{build}-\code{PL}}
\newcommand{\tcparaxs}{\code{TC}-\code{build}-\code{PL}\xspace}
\newcommand{\tcquery}{\code{TC}-\code{query}}
\newcommand{\tcqueryxs}{\code{TC}-\code{query}\xspace}
\newcommand{\tcidx}{\code{TC}-\code{Index}\xspace}
\newcommand{\topchain}{\code{TopChain}}
\newcommand{\topchainxs}{\code{TopChain}\xspace}

\newcommand{\mypath}{\mathcal{P}}
\newcommand{\mywedge}{\mathcal{W}}
\newcommand{\idx}{\code{TBP}-\code{Index}\xspace}
\newcommand{\idxplus}{\code{TBP}-\code{Index+}\xspace}
\newcommand{\tbp}{\code{TBP}}
% \newcommand{\online}{\code{OnlineReach}}
% \newcommand{\onlinexs}{\code{OnlineReach}\xspace}
% \newcommand{\onlineplus}{\code{OnlineReach}$^*$}
% \newcommand{\onlineplusxs}{\code{OnlineReach}$^*$\xspace}
% \newcommand{\monlineplus}{\code{MOnlineReach}$^*$}
% \newcommand{\monlineplusxs}{\code{MOnlineReach}$^*$\xspace}
\newcommand{\online}{\code{OReach}}
\newcommand{\onlinexs}{\code{OReach}\xspace}
% \newcommand{\onlineplus}{\code{OReach}$^*$}
% \newcommand{\onlineplusxs}{\code{OReach}$^*$\xspace}
\newcommand{\onlineplus}{\code{OReach}}
\newcommand{\onlineplusxs}{\code{OReach}\xspace}
\newcommand{\newonline}{\code{OReach}$^+$}
\newcommand{\newonlinexs}{\code{OReach}$^+$\xspace}
% \newcommand{\monlineplus}{\code{MOReach}$^*$}
% \newcommand{\monlineplusxs}{\code{MOReach}$^*$\xspace}
\newcommand{\monlineplus}{\code{MOReach}}
\newcommand{\monlineplusxs}{\code{MOReach}\xspace}
\newcommand{\tbpquery}{\code{TBP}-\code{query}}
\newcommand{\tbpqueryxs}{\code{TBP}-\code{query}\xspace}
\newcommand{\tbpnaive}{\code{TBP}-\code{build}}
\newcommand{\tbpnaivexs}{\code{TBP}-\code{build}\xspace}
\newcommand{\tbptp}{\code{TBP}-\code{build}$^+$}
\newcommand{\tbptpxs}{\code{TBP}-\code{build}$^+$\xspace}
\newcommand{\tbppr}{\code{TBP}-\code{build}$^{++}$}
\newcommand{\tbpprxs}{\code{TBP}-\code{build}$^{++}$\xspace}

\newcommand{\tbpplus}{\code{TBP}-\code{build}$^*$}
\newcommand{\tbpplusxs}{\code{TBP}-\code{build}$^*$\xspace}
\newcommand{\tbppara}{\code{TBP}-\code{build}$^*$-\code{PL}}
\newcommand{\tbpparaxs}{\code{TBP}-\code{build}$^*$-\code{PL}\xspace}
\newcommand{\phaseI}{\kw{Phase}\xspace\kw{I}}
% \newcommand{\phaseI}{\code{Phase}\xspace\code{I}}
\newcommand{\phaseII}{\kw{Phase}\xspace\kw{II}}
\newcommand{\caseI}{\kw{Case}\xspace\kw{I}}
\newcommand{\caseII}{\kw{Case}\xspace\kw{II}}
\newcommand{\caseIII}{\kw{Case}\xspace\kw{III}}
\newcommand{\pholder}{\boldsymbol{\cdot}}


% \newcommand{\inifunc}{\mathcal{L}}
% \newcommand{\Matching}{\code{Matching}\xspace}
% \newcommand{\Denominator}{\code{Denominator}\xspace} 
% \newcommand{\argmax}{\mathop{\mathrm{argmax}}}
% \newcommand{\normopr}{\Omega}
% \newcommand{\mappingopr}{\mathcal{M}}
% \newcommand{\lparam}{(1-{w^+}-{w^-})}
% \newcommand{\outparam}{w^+}
% \newcommand{\inparam}{w^-}
	

==> sections/acknowledgements.tex <==
This work was partially supported by 
Australian Research Council (ARC) Discovery Project DP230101534, Australian Research Council Future Fellowship FT210100303.
This work was also supported in part by 
NSFC under Grant 62102341, Basic and Applied Basic Research Fund in Guangdong Province under Grant 2022A1515010166, Shenzhen Science and Technology Program under Grants JCYJ20220530143602006 and ZDSYS20211021111415025, and Guangdong Talent Program under Grant 2021QN02X826. 
The authors would like to thank the anonymous reviewers for providing constructive feedback and valuable suggestions.
